Interfacial assembly of anisotropic core-shell and hollow microgels

Microgels, cross-linked polymers with submicrometer size, are ideal soft model systems. While spherical microgels have been studied extensively, anisotropic microgels have been hardly investigated. In this study, we compare the interfacial deformation and assembly of anisotropic core-shell and hollow microgels. The core-shell microgel consists of an elliptical core of hematite covered with a thin silica layer and a thin shell made of PNiPAM. The hollow microgels were obtained after a two step etching procedure of the inorganic core. The behavior of these microgels at the oil-water interface was investigated in a Langmuir Blodgett trough combined with ex-situ AFM. First, the influence of the architecture of anisotropic microgels on their spreading at the interface was investigated experimentally and by dissipative particle dynamic simulations. Hereby, the importance of the local shell thickness on the lateral and longitudinal interfacial deformation was highlighted as well as the differences between the core-shell and hollow architectures. The shape of the compression isotherms as well as the dimensions, ordering and orientation of the microgels at the different compressions were analysed. Due to their anisotropic shape and stiffness, both anisotropic microgels were found to exhibit significant capillary interactions with a preferential side-to-side assembly leading to stable microgel clusters at low interfacial coverage. Such capillary interactions were found to decrease in the case of the more deformable hollow anisotropic microgels. Consequently, anisotropic hollow microgels were found to distribute more evenly at high surface pressure compared to stiffer core-shell microgels. Our findings emphasize the complex interplay between the colloid design, anisotropy and softness on the interfacial assembly and the opportunities it thus offers to create more complex ordered interfaces.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
